Euclid preparation: IX. EuclidEmulator2 -- Power spectrum emulation with massive neutrinos and self-consistent dark energy perturbations

We present a new, updated version of the EuclidEmulator (called EuclidEmulator2), a fast and accurate predictor for the nonlinear correction of the matter power spectrum. Percent-level accurate emulation is now supported in the eight-dimensional parameter space of $w_0w_a$CDM$+\sum m_\nu$models between redshift $z=0$ and $z=3$ for spatial scales within the range 0.01 $h$/Mpc $\leq k \leq$ 10 $h$/Mpc. In order to achieve this level of accuracy, we have had to improve the quality of the underlying N-body simulations used as training data: (1) we use self-consistent linear evolution of non-dark matter species such as massive neutrinos, photons, dark energy and the metric field, (2) we perform the simulations in the so-called N-body gauge, which allows one to interpret the results in the framework of general relativity, (3) we run over 250 high-resolution simulations with $3000^3$ particles in boxes of 1 (Gpc/$h$)${}^3$ volumes based on paired-and-fixed initial conditions and (4) we provide a resolution correction that can be applied to emulated results as a post-processing step in order to drastically reduce systematic biases on small scales due to residual resolution effects in the simulations. We find that the inclusion of the dynamical dark energy parameter $w_a$ significantly increases the complexity and expense of creating the emulator. The high fidelity of EuclidEmulator2 is tested in various comparisons against N-body simulations as well as alternative fast predictors like Halofit, HMCode and CosmicEmu. A blind test is successfully performed against the Euclid Flagship v2.0 simulation. Nonlinear correction factors emulated with EuclidEmulator2 are accurate at the level of 1% or better for 0.01 $h$/Mpc $\leq k \leq$ 10 $h$/Mpc and $z\leq3$ compared to high-resolution dark matter only simulations. EuclidEmulator2 is publicly available at https://github.com/miknab/EuclidEmulator2 .

==> Chapters/xxx_DataProducts.tex <==
\section{Data Products}
\subsection{Matter power spectrum and its nonlinear correction}
The matter power spectrum is one of the key quantities in the study of cosmic large scale structure and its evolution. Our N-body simulations have baryons only in the background and do not evolve them. Fully nonlinear contributions are hence coming solely from dark matter particles, however, as described in \autoref{sec:theory} and \autoref{sec:NbodySims}, perturbations in the photon, neutrino, dark energy and metric fields are evolved at the linear level. The nonlinear correction factor (often referred to as the nonlinear boost factor) is theoretically defined by:
\begin{equation}
    B_{\rm th}(k,z)=\frac{P_{\rm nonlin}(k,z)}{P_{\rm lin}(k,z)}    
\end{equation}
Thanks to the fact that with our new simulation pipeline for the first time we can achieve N-body results that are fully consistent with \gls{GR} and hence reproduce linear theory very accurately at large scales at all redshifts, we can actually compute the nonlinear correction factor as defined by theory. Previously in \citet{Knabenhans2019EuclidSpectrum}, we were still forced to use the standard procedure of computing the nonlinear correction by rescaling the initial conditions to the redshift of interest. However, in presence of massive neutrinos it is not entirely clear how to perform this rescaling in detail. That this approach works very well is e.g. visible in \autoref{fig:VolConv_Pk}.

Further, we have shown in \citet{Knabenhans2019EuclidSpectrum} that emulating the logarithm of the boost factor yields more accurate predictions. Hence the final target value to predict is $\ln(B(k,z))$.

\subsection{Velocity power spectrum}
In order to make {\EEtwo} useful for parameter forcasting exercises, one needs to make sure that predictions by the emulator can be compared to observable quantities. The raw matter power spectrum is not observable due to various effects such as galaxy bias, \gls{RSDs},  the \gls{AP} effect and others (see e.g. \citealt{Sprenger2019CosmologyCitations} and references therein). While emulating all these correction factors clearly is beyond the scope of this paper, we decide to emulate the nonlinear velocity power spectrum $P_{\rm v}(k,z)$ which is a key ingredient to catch \gls{RSDs}. 

\subsubsection{Bispectrum}
The bispectrum is a crucial quantity when studying nonlinear structure formation: For a perfectly Gaussian random field the bispectrum vanishes and hence a non-vanishing bispectrum naturally carries information about non-Gaussianity. Assuming that the matter density field in the Universe is initially Gaussian, this translates into a measure for nonlinear evolution.

\subsection{Halo Mass Function}
\subsection{Density field}
Emulating the density field directly has the clear advantage that many quantities can be derived from it in a post-processing step. However, it is beyond our possibilities to provide the data for multiple realizations per cosmology, not just because our computational budget is not big enough, but also because the corresponding data is of the order of a few terrabytes per cosmology. We hence provide a density field emulator for one single realization. Any derived quantity will hence be affected non-negligibly by cosmic sampling variance.




